Zipping Segment Trees

Stabbing queries in sets of intervals are usually answered using segment trees. A dynamic variant of segment trees has been presented by van Kreveld and Overmars, which uses red-black trees to do rebalancing operations. This paper presents zipping segment trees - dynamic segment trees based on zip trees, which were recently introduced by Tarjan et al. To facilitate zipping segment trees, we show how to uphold certain segment tree properties during the operations of a zip tree. We present an in-depth experimental evaluation and comparison of dynamic segment trees based on red-black trees, weight-balanced trees and several variants of the novel zipping segment trees. Our results indicate that zipping segment trees perform better than rotation-based alternatives.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages

\usepackage{scrhack}

\usepackage[ngerman,main=american]{babel}

\usepackage{calc}

\usepackage{printlen}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Indentation

\newlength{\myparindent}
\newlength{\myparskip}
\setlength{\myparindent}{1em}
\setlength{\myparskip}{0em}

\setlength{\parindent}{\myparindent}
\setlength{\parskip}{\myparskip}
\setlength{\parskip}{0pt plus1pt minus0pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Colors

\usepackage[usenames,dvipsnames,table]{xcolor}

% Thesis colors
\definecolor{thesisblue}         {rgb}{0.337, 0.592, 0.773}
\definecolor{thesisblue-dark}    {rgb}{0.212, 0.471, 0.655}
\definecolor{thesisblue-light}   {rgb}{0.490, 0.710, 0.867}
\definecolor{thesisblue-vlight}  {rgb}{0.871, 0.937, 0.988}

\definecolor{thesisred}          {rgb}{0.776, 0.357, 0.396}
\definecolor{thesisred-dark}     {rgb}{0.663, 0.235, 0.271}
\definecolor{thesisred-light}    {rgb}{0.867, 0.502, 0.533}
\definecolor{thesisred-vlight}   {rgb}{0.984, 0.871, 0.878}

\definecolor{thesisgreen}        {rgb}{0.337, 0.765, 0.235}
\definecolor{thesisgreen-dark}   {rgb}{0.267, 0.612, 0.184}
\definecolor{thesisgreen-light}  {rgb}{0.443, 0.871, 0.341}
\definecolor{thesisgreen-vlight} {rgb}{0.710, 0.984, 0.643}

\definecolor{thesisyellow}       {rgb}{0.808, 0.659, 0.263}
\definecolor{thesisyellow-dark}  {rgb}{0.667, 0.529, 0.180}
\definecolor{thesisyellow-light} {rgb}{0.898, 0.765, 0.412}
\definecolor{thesisyellow-vlight}{rgb}{0.992, 0.933, 0.776}

\definecolor{black}              {rgb}{0,0,0}
\definecolor{black70}            {rgb}{0.30,0.30,0.30}
\definecolor{black50}            {rgb}{0.50,0.50,0.50}
\definecolor{black30}            {rgb}{0.70,0.70,0.70}
\definecolor{black15}            {rgb}{0.85,0.85,0.85}
\definecolor{black7}             {rgb}{0.95,0.95,0.95}

% Set major colors
\colorlet{primarycolor-dark}      {thesisblue-dark}
\colorlet{primarycolor}           {thesisblue}
\colorlet{primarycolor-light}     {thesisblue-light}
\colorlet{primarycolor-vlight}    {thesisblue-vlight}
\colorlet{secondarycolor-dark}    {thesisred-dark}
\colorlet{secondarycolor}         {thesisred}
\colorlet{secondarycolor-light}   {thesisred-light}
\colorlet{secondarycolor-vlight}  {thesisred-vlight}

\colorlet{stroke1}                {primarycolor-dark}
\colorlet{stroke2}                {secondarycolor-dark}

% Set document colors
\colorlet{captionlabel}{black}
\colorlet{footerpagenr}{black}
\colorlet{footerchapter}{stroke1}
\colorlet{footerchaptername}{black}
\colorlet{footersection}{stroke1}
\colorlet{footersectionname}{black}
\colorlet{chapternumber}{stroke1}
\colorlet{sectiontitlenumber}{black}
\colorlet{sectiontitle}{black}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ...

\newlength{\tmpa}
\newlength{\tmpb}
\newlength{\tmpc}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Size and position of the text body

\newlength{\mybodywidth}
\newlength{\mybodyheight}
\newlength{\myoutermargin}
\newlength{\mytopmargin}
\setlength{\mybodywidth}{132.5mm}
\setlength{\mybodyheight}{195mm}
\setlength{\myoutermargin}{51.8mm}%+5mm}
\setlength{\mytopmargin}{38mm}

\newlength{\myinnermargin}
\newlength{\mybottommargin}
\setlength{\myinnermargin}{\paperwidth-\mybodywidth-\myoutermargin}
\setlength{\mybottommargin}{\paperheight-\mybodyheight-\mytopmargin}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Position of the cut marks

\newlength{\cutmarktop}
\newlength{\cutmarkbottom}
\newlength{\cutmarkinner}
\newlength{\cutmarkouter}

\setlength{\cutmarktop}{7mm}
\setlength{\cutmarkbottom}{7mm}
\setlength{\cutmarkinner}{0mm}
\setlength{\cutmarkouter}{7mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Position of the head and foot

\newcommand{\goldenratio}{1.618}

\newlength{\myheadsep} % distance from header to body
\setlength{\myheadsep}{(\mytopmargin-\cutmarktop) -
  (\mytopmargin-\cutmarktop) / \real{\goldenratio} - 1ex}

\newlength{\myfootskip} % distance from body to footer
\setlength{\myfootskip}{(\mybottommargin-\cutmarkbottom) /
  \real{\goldenratio} - 1ex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Margin position and width

\newlength{\mymargininnersep} % distance between margin and body
\newlength{\mymarginoutersep} % distance between margin and paper edge
\newlength{\mymarginwidth} % width of the margin
\setlength{\mymargininnersep}{7mm}
\setlength{\mymarginoutersep}{12mm}
\setlength{\mymarginwidth}{\myoutermargin - \mymargininnersep -
  \mymarginoutersep - \cutmarkouter}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Applying the geometry

\usepackage[
paper=a4paper,
width=\mybodywidth,
height=\mybodyheight,
outer=\myoutermargin,
top=\mytopmargin,
headsep=\myheadsep,
footskip=\myfootskip,
marginparsep=\mymargininnersep,
marginparwidth=\mymarginwidth,
% showframe
]{geometry}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Printing crop marks

\usepackage{tikz}
\setlength{\tmpa}{1mm}
\newcommand{\cropmarkeven}{%
  \begin{tikzpicture}[overlay,remember picture]%
    \node [inner sep=0,outer sep=0, anchor=north west] at (current
    page.north west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (\cutmarkouter,0mm) -- (\cutmarkouter,-\cutmarktop+\tmpa);%
        \draw (0mm,-\cutmarktop) -- (\cutmarkouter-\tmpa,-\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=north east] at (current
    page.north east) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (0mm,-\cutmarktop) -- (-\cutmarkouter+\tmpa,-\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=south west] at (current
    page.south west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (\cutmarkouter,0mm) -- (\cutmarkouter,\cutmarktop-\tmpa);%
        \draw (0mm,\cutmarktop) -- (\cutmarkouter-\tmpa,\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=south east] at (current
    page.south east) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (0mm,\cutmarktop) -- (-\cutmarkouter+\tmpa,\cutmarktop);%
      \end{tikzpicture}%
    };%
  \end{tikzpicture}
}
\newcommand{\cropmarkodd}{%
  \begin{tikzpicture}[overlay,remember picture]%
    \node [inner sep=0,outer sep=0, anchor=north west] at (current
    page.north west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (0mm,-\cutmarktop) -- (\cutmarkouter-\tmpa,-\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=north east] at (current
    page.north east) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (-\cutmarkouter,0mm) -- (-\cutmarkouter,-\cutmarktop+\tmpa);%
        \draw (0mm,-\cutmarktop) -- (-\cutmarkouter+\tmpa,-\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=south west] at (current
    page.south west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (0mm,\cutmarktop) -- (\cutmarkouter-\tmpa,\cutmarktop);%
      \end{tikzpicture}%
    };%
    \node [inner sep=0,outer sep=0, anchor=south east] at (current
    page.south east) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw (-\cutmarkouter,0mm) -- (-\cutmarkouter,\cutmarktop-\tmpa);%
        \draw (0mm,\cutmarktop) -- (-\cutmarkouter+\tmpa,\cutmarktop);%
      \end{tikzpicture}%
    };%
  \end{tikzpicture}
}

\usepackage{everypage}
\usepackage[strict]{changepage}

\newcommand{\showcropmarks}{%
  \AddEverypageHook{%
    \checkoddpage%
    \ifoddpage%
    \cropmarkodd%
    \else%
    % \cropmarkeven%
    \fi%
  }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Header and footer format

\usepackage{fancyhdr}
\pagestyle{fancy} 

\fancypagestyle{plain}{%
  \fancyhf{} % clear header and footer

  % no header/footer line
  \renewcommand{\headrulewidth}{0pt}
  \renewcommand{\footrulewidth}{0pt}

  % set distances
  \fancyheadoffset[EL]{\myoutermargin}
  \fancyheadoffset[OR]{\myoutermargin}
  \fancyfootoffset[EL]{\myoutermargin}
  \fancyfootoffset[OR]{\myoutermargin}

  % page numbers
  \fancyfoot[EL]{%
    {\color{stroke1}\rule{\myoutermargin-\mymargininnersep}{0.5mm}}\\
    \begin{minipage}[b]{\myoutermargin-\mymargininnersep}%
      \raggedleft\color{footerpagenr}\textbf{\thepage}%
    \end{minipage}%
  }
  \fancyfoot[OR]{%
    {\color{stroke1}\rule{\myoutermargin-\mymargininnersep}{0.5mm}}\\
    \begin{minipage}[b]{\myoutermargin-\mymargininnersep}%
      \raggedright\color{footerpagenr}\textbf{\thepage}%
    \end{minipage}%
  }
}

\fancypagestyle{content}{%
  % use default page numbering
  \pagestyle{plain}

  % define header
  \renewcommand{\chaptermark}[1]{%
    \markboth{%
      \small\textsf{\color{footerchaptername}##1}%
    }{}%
  }
  \renewcommand{\sectionmark}[1]{%
    \markright{%
      \small\textsf{\color{footersectionname}##1}%
    }%
  } 
  \fancyhead[EL]{%
    \begin{minipage}[b]{\myoutermargin-\mymargininnersep}%
      \small%
      \raggedleft\textsf{\textbf{\color{footerchapter}\chaptername\ \thechapter}}
    \end{minipage}%
    \hspace{\mymargininnersep}\leftmark%
  }
  \fancyhead[OR]{%
    \rightmark\hspace{\mymargininnersep}%
    \begin{minipage}[b]{\myoutermargin-\mymargininnersep}%
      \small%
      \raggedright\textsf{\textbf{\color{footersection}Section\ \thesection}}
    \end{minipage}%
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caption format

\usepackage{caption}
\captionsetup{
  font=small,
  labelfont={bf,sf,color=captionlabel},
  format=plain,
  singlelinecheck=off
  %tableposition=top
}

\usepackage{floatrow}
\floatsetup[table]{capposition=top}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% part format

\usepackage[noindentafter,explicit]{titlesec}

\assignpagestyle{\part}{empty}
\titleformat{\part}
[display]
{\Huge\sffamily}%
{}%
{-2\baselineskip}%
{%
  \setlength{\tmpa}{0.618\paperwidth}%
  \setlength{\tmpb}{0.382\paperheight}%
  \begin{tikzpicture}[overlay,remember picture]%
    \node [inner sep=0,outer sep=0, anchor=north] at (current
    page.north west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw[color=stroke1, line width=0.7mm] (\tmpa,0) -- (\tmpa,-\tmpb);%
      \end{tikzpicture}%
    };%
    \node (align) [align=right, below=\tmpb-2ex, inner sep=0, outer
    sep=0, anchor=north west] at (current page.north west){%
      \hspace{\tmpa}\hspace{0.5em}\partname\ \thepart\\[1ex]%
      \color{stroke1}#1%
    };%
  \end{tikzpicture}%
}%
[]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Chapter format

\assignpagestyle{\chapter}{plain}
\titlespacing{\chapter}{0mm}{0mm}{0mm}
\titleformat{\chapter}
[display]%
{\sffamily\color{stroke1}\huge}% format
{}% label
{0pt}% sep
{%
  \begin{tikzpicture}[overlay,remember picture]%
    \node [right=\myinnermargin,below=\mytopmargin, inner sep=0, outer
    sep=0, anchor=north west] (numbernode) at (current page.north west){%
      \hspace{\myinnermargin}%
      \sffamily\fontsize{60}{60}\selectfont%
      \color{chapternumber}%
      \thechapter%
    };%
    \node [inner sep=0,outer sep=0, anchor=north west] at (numbernode.south west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw[color=stroke1, line width=0.7mm] (\myinnermargin,-1ex) -- (\paperwidth,-1ex);%
      \end{tikzpicture}%
    };%
    \node (align) [align=right, right=\myinnermargin+\mybodywidth, inner sep=0, outer sep=0,
    anchor=east] at (numbernode.west) {%
      #1%
    };%
  \end{tikzpicture}%
}% before-code
[\bigskip]% after-code

\titleformat{name=\chapter,numberless}
[display]%
{\sffamily\color{stroke1}\huge}% format
{}% label
{0pt}% sep
{%
  \begin{tikzpicture}[overlay,remember picture]%
    \node [right=\myinnermargin,below=\mytopmargin, inner sep=0, outer
    sep=0, anchor=north west] (numbernode) at (current page.north west){%
      \hspace{\myinnermargin}%
      \sffamily\fontsize{60}{60}\selectfont%
      \color{white}%
      \thechapter%
    };%
    \node [inner sep=0,outer sep=0, anchor=north west] at (numbernode.south west) {%
      \begin{tikzpicture}[overlay,remember picture]%
        \draw[color=stroke1, line width=0.7mm] (\myinnermargin,-1ex) -- (\paperwidth,-1ex);%
      \end{tikzpicture}%
    };%
    \node (align) [align=left, right=\myinnermargin, inner sep=0, outer sep=0,
    anchor=south west] at (numbernode.south west) {%
      #1%
    };%
  \end{tikzpicture}%
}% before-code
[\bigskip]% after-code


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section format

% \titleformat{\section}%
% [block]%
% {\Large\bfseries\sffamily}%
% {\color{sectiontitlenumber}\thesection\hspace{0.5em}}%
% {0pt}%
% {\color{sectiontitle}\raggedright}%
% []


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Subsection format

% \titleformat{\subsection}%
% [block]%
% {\large\bfseries\sffamily}%
% {\color{sectiontitlenumber}\thesubsection\hspace{0.5em}}%
% {0pt}%
% {\color{sectiontitle}\raggedright}%
% []


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Paragraph format

\titleformat{\paragraph}%
[runin]%
{\bfseries\sffamily}%
{}%
{0pt}%
{#1.}%
[]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Biblatex and CV packages

\usepackage[utf8]{inputenc}

\usepackage{currvita}
\usepackage{csquotes}
\usepackage[
style=alphabetic,
%style=trad-alpha,
%style=numeric,
maxnames=100,
backend=biber,
defernumbers,
safeinputenc,
backref=true,
backrefstyle=none,
sortcites
]{biblatex}

\patchcmd{\bibsetup}{\interlinepenalty=5000}{\interlinepenalty=10000}{}{}

% Set up back references.
\DefineBibliographyStrings{english}{%
  backrefpage = {cited on page}, % originally "cited on page"
  backrefpages = {cited on pages}, % originally "cited on pages"
}

\DeclareFieldFormat{pagerefformat}{#1}
% \DeclareFieldFormat{pagerefformat}{\small\color{stroke1}\mkbibemph{{#1}}}

\renewbibmacro*{pageref}{%
  \addperiod%
  \iflistundef{pageref}%
    {}%
    {\newline\footnotesize\printtext[pagerefformat]{%
       \ifnumgreater{\value{pageref}}{1}%
         {\bibstring{backrefpages}\ppspace}%
     {\bibstring{backrefpage}\ppspace}%
       \printlist[pageref][-\value{listtotal}]{pageref}\addperiod}}}

% Set up bibliography layout.
\DeclareNumChars*{:}
\renewcommand{\intitlepunct}{\addspace}
\renewcommand{\multicitedelim}{\addcomma\space}

\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}

\renewbibmacro*{volume+number+eid}{
  \printfield{volume}
  \iffieldundef{number}{}{\addcolon}%
  \printfield{number}
  \setunit*{\addcomma\space}
  \printfield{eid}
}

\renewbibmacro*{editor+others}{%
  \ifboolexpr{
    test \ifuseeditor
    and
    not test {\ifnameundef{editor}}
  }
    {\printnames{editor}%
     \setunit{\space}%
     \usebibmacro{editor+othersstrg}%
     \clearname{editor}}
    {}}


\addbibresource{references.bib}

\DeclareFieldFormat[article]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inproceedings]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[thesis]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[book]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[unpublished]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[report]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inbook]{chapter}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inbook]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat{editortype}{\mkbibparens{#1}}
\DeclareFieldFormat[misc]{title}{\textbf{\color{stroke1}#1}}

\DefineBibliographyStrings{english}{%
  editor  = {editor},
  editors = {editors},
  page    = {page},
  pages   = {pages},
  volume  = {volume},
}

\newtoggle{authorend}
\togglefalse{authorend}

\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{bytranslator+others}%
  \newunit\newblock
  \printfield{version}%
  \newunit\newblock
  \usebibmacro{journal}
  \setunit{\addnbspace}
  \usebibmacro{volume+number+eid}
  \newunit
  \usebibmacro{byeditor+others}%
  \newunit
  \usebibmacro{note+pages}%
  \setunit{\addcomma\space}
  \printfield{year}
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{issn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

\DeclareBibliographyDriver{inbook}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \printfield{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{in:}%
  \usebibmacro{maintitle+booktitle}%
  \newunit\newblock
  \usebibmacro{byeditor+others}%
  \newunit\newblock
  \printfield{edition}%
  \iffieldundef{volume}
  {\setunit{\addcomma\space}}
  {  \newunit\printfield{volume}%
    \printfield{part}\space\bibstring{ofseries}\space\printfield{series}\setunit{\addcomma\space}}%
  \printfield{pages}
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \usebibmacro{publisher+location+date}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

\DeclareBibliographyDriver{book}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/editor+others/translator+others}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{maintitle+title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{byeditor+others}%
  \newunit\newblock
  \printfield{edition}%
  \newunit
  \iffieldundef{volume}
  {\setunit{\addcomma\space}}
  {  \newunit\printfield{volume}%
    \printfield{part}\space\bibstring{ofseries}\space\printfield{series}\setunit{\addcomma\space}}%
  %
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \usebibmacro{publisher+location+date}%
  \newunit
  \iflistundef{location}%
  {\setunit*{\addcomma\space}}%
  {\setunit*{\addcomma\space}}%
  \printlist{location}%
  {}
  \newunit
  \usebibmacro{chapter+pages}%
  \newunit
  \printfield{pagetotal}%
  \newunit\newblock
  \iftoggle{bbx:isbn}%
  {\printfield{isbn}}%
  {}
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \newunit\newblock
  \usebibmacro{pageref}%
  \usebibmacro{finentry}
}

\DeclareBibliographyDriver{inproceedings}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{in:}%
  \usebibmacro{maintitle+booktitle}%
  \newunit\newblock
  \usebibmacro{event+venue+date}%
  \newunit\newblock
  \usebibmacro{byeditor+others}%
  \newunit\newblock
  \iffieldundef{volume}
  {}
  {\printfield{volume}%
    \printfield{part}\space\bibstring{ofseries}}
  \printfield{series}%
  \newunit\newblock
  \usebibmacro{chapter+pages}%
  \iflistundef{publisher}%
  {\setunit{\addcomma\space}}%
  {\newunit\newblock}%
  \usebibmacro{publisher+location+date}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

\DeclareBibliographyDriver{thesis}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \printfield{type}%
  \newunit
  \usebibmacro{institution+location+date}%
  \newunit\newblock
  \usebibmacro{chapter+pages}%
  \newunit
  \printfield{pagetotal}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author}}{}%
}

\DeclareBibliographyDriver{misc}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \printfield{type}%
  \space
  \printfield{number}%
  \newunit\newblock
  \usebibmacro{institution+location+date}%
  \newunit
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

% Copied from numeric.cbx to imitate numerical citations.
\providebool{bbx:subentry}
\newbibmacro*{citenum}{%Note: the original macro was called "cite". I did not redefine "cite", but instead defined a new macro "citenum", because the author-year citations use the "cite" macro too. "\renewbibmacro*{cite}" would have caused all the author-year citations to become numeric too.
  \printtext[bibhyperref]{%If you ever want to use hyperref
    \printfield{prefixnumber}%
    \printfield{labelnumber}%
    \ifbool{bbx:subentry}
    {\printfield{entrysetcount}}
    {}}}

% Copied from numeric.cbx to define a new numeric citation command for @online entries.
\DeclareCiteCommand{\conline}[\mkbibbrackets]
{\usebibmacro{prenote}}
{\usebibmacro{citeindex}%
  \usebibmacro{citenum}}%Note: this was originally "cite" but I changed it to "citenum" to avoid clashes with the author-year style.
{\multicitedelim}
{\usebibmacro{postnote}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other packages 

\usepackage[T1]{fontenc}

\usepackage[final]{microtype}

\usepackage{amsmath}

\usepackage{amssymb}

\usepackage{amsthm}

\usepackage{thmtools}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% I really want \pfun from:
% \usepackage{oz}
%
% but that package is braindead and does things like
%
% \let \prod  \times
%
% or
%
% \let \num   \integer
%
% So. Brace for my own \pfun:
\makeatletter
\def\@oz_p#1{\mathrel{\ooalign{\hfil$\mapstochar\mkern 5mu$\hfil\cr$#1$}}}
\def \pfun  {\@oz_p\rightarrow}
\makeatother

\usepackage[
%hidelinks,
%ocgcolorlinks=true,
%colorlinks=true,
%linkcolor=stroke1,
%urlcolor=stroke1,
%citecolor=stroke2,
linkbordercolor=primarycolor-vlight,
urlbordercolor=primarycolor-vlight,
citebordercolor=secondarycolor-vlight,
pdftex,
pdfauthor={Lukas Barth},
pdftitle={Scheduling Algorithms for the Smart Grid}
]{hyperref}

%\usepackage[ocgcolorlinks]{ocgx2}

\usepackage{graphicx}

\usepackage{paralist}

\usepackage{booktabs}

\usepackage{multirow}

\usepackage{makecell}

\usepackage{rotating}

\usepackage{xspace}

\usepackage[absolute,overlay]{textpos}

\usepackage[ttscale=.85]{libertine}

\usepackage[libertine,cmintegrals,cmbraces,vvarbb]{newtxmath}

\usepackage{timetravel}
\setCounters{theorem}

\usepackage{adjustbox}
\usepackage{hvfloat}

\usepackage{circledsteps}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notes
\usepackage[textsize=scriptsize]{todonotes}
\newcommand{\maybe}[1]{\todo[color=green]{#1}}
\newcommand{\finalize}[1]{\todo[color=yellow]{#1}}

\usepackage{accents}

\usepackage{mathtools}

\usepackage{subcaption}
\captionsetup[subfigure]{justification=centering}

\usepackage[innercaption]{sidecap}
\columnsep=\mymargininnersep

\usepackage{pgfplots}
\usepackage{filecontents}
\pgfplotsset{compat=1.9}
\usepgfplotslibrary{external} 
\tikzexternalize[prefix=tikz/]
\tikzexternaldisable

\usepackage{environ}
\makeatletter
\newsavebox{\measure@tikzpicture}
\NewEnviron{scaletikzpicturetowidth}[1]{%
  \def\tikz@width{#1}%
  \def\tikzscale{1}\begin{lrbox}{\measure@tikzpicture}%
  \BODY
  \end{lrbox}%
  \pgfmathparse{#1/\wd\measure@tikzpicture}%
  \edef\tikzscale{\pgfmathresult}%
  \BODY
}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algorithm stuff

\usepackage[ruled, vlined, linesnumbered, noend]{algorithm2e}
%\DontPrintSemicolon

%%%%%%% Highlighting of code parts
%define a marking command
\newcommand*{\tikzmk}[1]{\tikz[remember picture,overlay,] \node (#1) {};\ignorespaces}
%define a boxing command, argument = colour of box
%\newcommand{\boxit}[1]{\tikz[remember picture,overlay]{\node[yshift=3pt,fill=#1,opacity=.25,fit={(A)($(B)+(.95\linewidth,.8\baselineskip)$)}] {};}\ignorespaces}
\newcommand{\boxit}[1]{\tikz[remember picture,overlay]{\node[yshift=4pt,fill=#1,opacity=.25,fit={(A)(B)}] {};}\ignorespaces}

%%%%%%%%%%%%%%%%%%%%% Begin of the Zündorf-Fix
\makeatletter
\renewcommand{\SetKwInOut}[2]{%
\sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
\expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
\newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
\sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
\else% else keep the larger dimension
\ifdim\wd\algocf@inoutbox>\inoutsize%
\setlength{\inoutsize}{\wd\algocf@inoutbox}%
\sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
\fi%
\fi% the dimension of the box is now defined.
\algocf@newcommand{#1}[1]{%
\ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
\ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
{\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo:}}~##1\par}%
\algocf@linesnumbered% reset the numbering of the lines
\ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
}}%
\renewcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them,
\strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
\algocf@push{\skiprule}%        move to the right before the vertical rule
\hbox{\vrule\hspace{-0.4pt}%
\vtop{\algocf@push{\skiptext}%move the right after the rule
\vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
\algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
\nointerlineskip}% no vskip after
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End of the Zündorf-Fix

% \SetAlFnt{\small}
% \newcommand{\commentfont}[1]{{\color{black50}#1}}
% \newcommand{\kwfont}[1]{\texttt{\color{stroke1}#1}}
% \newcommand{\funcfont}[1]{\texttt{#1}}
% \newcommand{\datafont}[1]{\texttt{#1}}

% \SetCommentSty{commentfont}
% \SetKwSty{kwfont}
% \SetFuncSty{funcfont}
% \SetDataSty{datafont}

\SetKwFunction{FnRepair}{RepairDuringInsertion}
\SetKwFunction{FnInsert}{Insert}
\SetKwProg{Fn}{Function}{:}{}


% \makeatletter
% \newcommand{\setalgotoprulecolor}[1]{\colorlet{toprulecolor}{#1}}
% \let\old@algocf@pre@ruled\@algocf@pre@ruled
% \renewcommand{\@algocf@pre@ruled}{\textcolor{toprulecolor}{\old@algocf@pre@ruled}}

% \newcommand{\setalgobotrulecolor}[1]{\colorlet{bottomrulecolor}{#1}}
% \let\old@algocf@post@ruled\@algocf@post@ruled
% \renewcommand{\@algocf@post@ruled}{\textcolor{bottomrulecolor}{\old@algocf@post@ruled}}

% \renewcommand{\algocf@caption@ruled}{}
% \makeatother

% \setalgotoprulecolor{stroke1}
% \setalgobotrulecolor{stroke1}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorems

\theoremstyle{plain} %
\newtheorem{theorem}{Theorem}[chapter] %
\newtheorem{lemma}[theorem]{Lemma} %
\newtheorem{corollary}[theorem]{Corollary} %
\newtheorem{proposition}[theorem]{Proposition} %
\newtheorem{problem}{Problem} % TODO This is only used in a few papers
\newtheorem{definition}{Definition} %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Math Operators

\DeclareMathOperator{\lca}{LCA} % Lowest common ancestor

\DeclareMathOperator{\lcs}{LCS}
\DeclareMathOperator{\slcs}{SLCS}
\DeclareMathOperator{\lc}{LC}
\DeclareMathOperator{\lcss}{LCSS}
\DeclareMathOperator{\mlcss}{MLCSS}

\DeclareMathOperator{\dom}{dom} % Domain of a partial function



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Index Generation
\usepackage{makeidx}
\makeindex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%% Term definition
%%
%% If you don't use the index (see above), remove the \index{#1} below!
\newcommand{\termdef}[2][*]{\ifthenelse{\equal{#1}{*}}%
  {\index{#2}\marginpar{\textsf{#2}}\emph{#2}}%
  {\ifthenelse{\equal{#1}{-}}
      {\index{#2}\marginpar{\textsf{#2}}}
        {\index{#1}\marginpar{\textsf{#1}}\emph{#2}}}%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% TikZ stuff

\usetikzlibrary{arrows}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{through}
\usetikzlibrary{intersections}
\usetikzlibrary{fit}
\usetikzlibrary{calc}
\tikzset{>=stealth'}

\tikzstyle{figure}=[font=\small]
\tikzstyle{vertex}=[circle, inner sep=0pt, minimum size=6pt, draw=black, fill=primarycolor-vlight]
\tikzstyle{bigvertex}=[vertex, minimum size=11pt]
\tikzstyle{chvertex}=[bigvertex]
\tikzstyle{textvertex}=[bigvertex, font=\footnotesize]
\tikzstyle{highlightedvertex}=[vertex, fill=secondarycolor-light]
\tikzstyle{highlightedchvertex}=[chvertex, fill=secondarycolor-light]
\tikzstyle{chargingstationvertex}=[double distance=1pt, fill=secondarycolor-light]
\tikzstyle{vertexhull}=[line width=14pt, rounded corners=2pt]
\tikzstyle{vertexhullboundary}=[vertexhull, line width=14.8pt]
\tikzstyle{chshortcutedges}=[edges, very thick, fill=secondarycolor, draw=primarycolor]
\tikzstyle{cell1vertex}=[vertex, fill=black30]
\tikzstyle{cell2vertex}=[vertex, fill=black15]
\tikzstyle{cell3vertex}=[vertex, fill=black50]
\tikzstyle{dualvertex}=[vertex, fill=secondarycolor-light]
\tikzstyle{dualtextvertex}=[textvertex, fill=secondarycolor-light]

\tikzstyle{edgelabel}=[inner sep=1pt, fill=white]
\tikzstyle{edges}=[shorten >=1pt, shorten <=1pt]
\tikzstyle{shortestpathedges}=[edges, line width=3pt, fill=secondarycolor-light, draw=secondarycolor-light]
\tikzstyle{internaledges}=[edges]
\tikzstyle{boundaryedges}=[internaledges, thick, densely dotted]
\tikzstyle{edgesbackground}=[line width=2pt, draw=white]
\tikzstyle{shortestpathedgesbackground}=[line width=4.5pt, draw=white]
\tikzstyle{dualedges}=[edges,thick,secondarycolor]

\tikzstyle{polygonalpath}=[thick, draw=primarycolor-dark]
\tikzstyle{polygonwindow}=[very thick,densely dotted]
\tikzstyle{polygonalarea}=[fill=primarycolor-vlight,draw=primarycolor-vlight]
\tikzstyle{polygon}=[polygonalpath, fill=primarycolor-vlight]
\tikzstyle{polygonhole}=[polygonalpath, fill=white]
\tikzstyle{outerpolygonalpath}=[thick]
\tikzstyle{triangulationedge}=[draw=black50]
\tikzstyle{point}=[circle, inner sep=0pt, minimum size=3pt, draw=black, fill=black]
\tikzstyle{specialpoint}=[point,fill=primarycolor]
\tikzstyle{minlinkpath}=[primarycolor,line width=2pt]
\tikzstyle{minlinkshortestpath}=[secondarycolor,very thick]
\tikzstyle{minlinkshortestpathmid}=[thesisyellow,very thick]
\tikzstyle{visibilitycone}=[primarycolor,very thick]
\pgfdeclareverticalshading{myshading}{100bp}{color(0bp)=(primarycolor-light); color(40bp)=(primarycolor-light); color(70bp)=(white); color(100bp)=(white)}
\pgfdeclareverticalshading{myshadingother}{100bp}{color(0bp)=(primarycolor-light); color(10bp)=(primarycolor-light); color(54bp)=(white); color(100bp)=(white)}
\tikzstyle{visibilityconearea}=[bottom color=primarycolor-light, top color=white,draw=white]
\tikzstyle{filledregionprimary}=[primarycolor-vlight]
\tikzstyle{filledregionsecondary}=[secondarycolor-vlight]

\tikzstyle{toplevelpartitionboundary}=[primarycolor-dark,line width=2.25pt]
\tikzstyle{botlevelpartitionboundary}=[secondarycolor-light, line width=1pt]
\tikzstyle{toplevelpartitiondescription}=[text=primarycolor-dark]
\tikzstyle{botlevelpartitiondescription}=[font=\footnotesize,text=secondarycolor-light]

\tikzstyle{function}=[draw=primarycolor,very thick,line cap=rect]
\tikzstyle{functionterm}=[text=primarycolor,edgelabel]
\tikzstyle{discontinuity}=[circle, inner sep=0pt, minimum size=3.5pt,very thick]
\tikzstyle{discontinuityblank}=[discontinuity,draw=primarycolor,fill=white]
\tikzstyle{discontinuityfilled}=[discontinuity,draw=primarycolor,fill=primarycolor]
\tikzstyle{plotgrid}=[color=black30,very thin,dash pattern=on 2pt off 1pt]
\tikzstyle{chargingfunction}=[function,draw=secondarycolor]
\tikzstyle{helperline}=[black]
\tikzstyle{breakpoint}=[fill,primarycolor,circle,inner sep=0pt,minimum size=3.5pt,very thick]

\tikzstyle{shrinkedface}=[thick,double distance=10pt,draw=primarycolor-dark, double=primarycolor-vlight]
\tikzstyle{reachablevertex}=[vertex, fill=white]
\tikzstyle{unreachablevertex}=[vertex, fill=black50]
\tikzstyle{passableedges}=[edges,black]
\tikzstyle{borderedges}=[edges,thick,densely dotted]
\tikzstyle{unreachableedges}=[edges,black]
\tikzstyle{reachableboundary}=[draw=primarycolor,line width=3pt]
\tikzstyle{unreachableboundary}=[draw=secondarycolor,line width=3pt]
\tikzstyle{visitededges}=[edges, line width=3pt, primarycolor-light]

\tikzstyle{plotpoint}=[fill=black,circle,inner sep=0pt,minimum size=3.5pt]
\tikzstyle{tangentline}=[shorten >=-20pt,shorten <= -15pt]

\tikzstyle{markSign} = [mark=*]
\tikzstyle{heuristicMarkSign} = [mark=o]
\tikzstyle{exactMarkSign} = [mark=*]
\tikzstyle{shortenLines} = [shorten <= 3.5pt,shorten >= 3.5pt]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\pgfplotsset{
  /pgfplots/legend line with mark/.style={
    legend image code/.code={
        \draw[##1,no markers,shorten >= 3.5pt,line width=1pt]
         plot coordinates {
         (0cm,0cm)
         (0.3cm,0cm)
        };
        \draw[##1,only marks,markSign,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
        };
        \draw[##1,no markers,shorten <= 3.5pt,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
         (0.6cm,0cm)
        };
    }
  }
}

\pgfplotsset{
  /pgfplots/legend line with heuristic mark/.style={
    legend image code/.code={
        \draw[##1,no markers,shorten >= 3.5pt,line width=1pt]
         plot coordinates {
         (0cm,0cm)
         (0.3cm,0cm)
        };
        \draw[##1,only marks,heuristicMarkSign,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
        };
        \draw[##1,no markers,shorten <= 3.5pt,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
         (0.6cm,0cm)
        };
    }
  }
}

\pgfplotsset{
  /pgfplots/legend line with exact mark/.style={
    legend image code/.code={
        \draw[##1,no markers,shorten >= 3.5pt,line width=1pt]
         plot coordinates {
         (0cm,0cm)
         (0.3cm,0cm)
        };
        \draw[##1,only marks,exactMarkSign,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
        };
        \draw[##1,no markers,shorten <= 3.5pt,line width=1pt]
         plot coordinates {
         (0.3cm,0cm)
         (0.6cm,0cm)
        };
    }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Float snafu
%\usepackage{pdflscape}
%\usepackage{afterpage}
\usepackage{rotating}
\usepackage{placeins}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Misc settings

\widowpenalties 2 10000 0
\clubpenalties 2 10000 0

\hyphenation{Karls-ruhe}
\hyphenation{Open-Access}

\setlength{\tabcolsep}{1.0ex}

\providecommand\phantomsection{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages from individual papers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ... from "A unified framework"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{eurosym} % load real euro symbol
\usepackage{siunitx} % use proper SI unit typesetting
\usepackage{longtable}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{dcolumn}
\usepackage{ragged2e}
\usepackage{colortbl}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{v}[1]{>{\PreserveBackslash\RaggedRight\hspace{0pt}}p{#1}}
  \usepackage{adjustbox}
\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}
\newcommand*\rottblhead{\multicolumn{1}{R{90}{1em}}}% no optional argument here, please!
\newcommand{\myparagraph}[1]{\paragraph{#1}\mbox{}\\}
\newcolumntype{a}{>{\columncolor{primarycolor-light}}v{0.4cm}}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ... from "Benchmark Dataset"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{cleveref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ... from "SWAG"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algortihm2E
% TODO an andere stelle in der preamble
\SetKw{KwOr}{or}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{FnRandomSelection}{randomSelection}
\SetKwFunction{FnFindDeletionEdgesForward}{findDeletionEdgesForward}
\SetKwFunction{FnFindDeletionEdgesBackward}{findDeletionEdgesBackward}
\SetKwFunction{FnPushFront}{pushFront}
\SetKwFunction{FnPushBack}{pushBack}
\SetKwFunction{FnPopFront}{popFront}
\SetKwFunction{FnMakeList}{makeList}
\SetKwFunction{FnMark}{mark}
\SetKwFunction{FnUnmark}{unmark}
\SetKwFunction{FnRecomputeLatestFinishFor}{computeLatestFinish}
\SetKwFunction{FnMax}{max}
\SetKwFunction{FnRemoveEdges}{removeEdges}
\SetKwFunction{FnInsertEdges}{insertEdges}
\SetKwFunction{FnDeterminePeakRange}{determinePeakRange}
\SetKwFunction{FnUnblockByDeletion}{unblockByDeletion}
\SetKwFunction{FnLeftShiftedSchedule}{leftShiftedSchedule}
\SetKwFunction{FnDeleteEdges}{deleteEdges}
\SetKwFunction{FnDelete}{delete}
\SetKwFunction{FnNotEmpty}{notEmpty}

% Parameters
\SetKwData{ParamDeletionTrials}{\underline{deletionTrials}}
\SetKwData{ParamDeletionMaxDepth}{\underline{deletionMaxDepth}}
\SetKwData{ParamUndermovePenalty}{\underline{undermovePenalty}}

% Style
\SetFuncArgSty{ensuremath}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For some reason, this cannot come too early, where all
% the other miscellaneous packages are included.
% Don't ask. LaTeX sucks.
%
\usepackage{bookmark}

%
% Switch between paper an thesis versions
%
\newcommand{\thesisonly}[1]{#1}
\newcommand{\paperonly}[1]{}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:

